Guided Meta-Policy Search

Reinforcement learning (RL) algorithms have demonstrated promising results on complex tasks, yet often require impractical numbers of samples since they learn from scratch. Meta-RL aims to address this challenge by leveraging experience from previous tasks so as to more quickly solve new tasks. However, in practice, these algorithms generally also require large amounts of on-policy experience during the meta-training process, making them impractical for use in many problems. To this end, we propose to learn a reinforcement learning procedure in a federated way, where individual off-policy learners can solve the individual meta-training tasks, and then consolidate these solutions into a single meta-learner. Since the central meta-learner learns by imitating the solutions to the individual tasks, it can accommodate either the standard meta-RL problem setting or a hybrid setting where some or all tasks are provided with example demonstrations. The former results in an approach that can leverage policies learned for previous tasks without significant amounts of on-policy data during meta-training, whereas the latter is particularly useful in cases where demonstrations are easy for a person to provide. Across a number of continuous control meta-RL problems, we demonstrate significant improvements in meta-RL sample efficiency in comparison to prior work as well as the ability to scale to domains with visual observations.

==> proof.tex <==
\section{Convergence Analysis Details}
\label{sec:theory}

We can perform a theoretical analysis of algorithm performance in a manner extremely similar to [cite PLATO]. Given a policy $\pi$, let us denote $d_{\pi}^t$ as the state distribution at time $t$ when executing policy $\pi$ from time $1$ to $t-1$. We can define the cost function $c(\bx_t, \bu_t) = - r(\bx_t, \bu_t)$ as a function of state $\bx_t$ and action $\bu_t$, with $c(\bx_t, \bu_t) \in [0,1]$ without loss of generality. 

Let us define $\pith + \nabla_k \pith = \pi_{\theta + \nabla_{\theta} \mathbb{E}_{\pith}[R_k]}$ as a shorthand for the policy which is obtained after the inner loop update for task $k$, with reward $R_k$ during meta-optimization. This will be used throughout the proof to represent a one-step update on a task indexed by $k$, essentially corresponding to policy gradient in the inner loop.  

We define the performance of a policy $\pith(\bu | \bx_t)$ over time horizon $T$:
\begin{align*}
J(\pi) = \sum_{t=1}^T \E_{\bx_t \sim d_{\pith}^t} [\E_{\bu_t \sim \pith(\bu | \bo_t)} [ c(\bx_t, \bu_t)]].
\end{align*}

This can be similarly extended to meta-updated policies as
\begin{align*}
J(\pith + \nabla_k \pith) = \sum_{t=1}^T \E_{\bx_t \sim d_{\pith + \nabla_k \pith}^t} [\E_{\bu_t \sim \pith + \nabla_k \pith} [ c(\bx_t, \bu_t)]].
\end{align*}

Let us define $J_t^k(\pi, \tilde{\pi})$ as the expected cost for task $k$ when executing $\pi$ for $t$ time steps, and then executing $\tilde{\pi}$ for the remaining $T-t$ time steps, and let us similarly define $Q_t^k(\bx, \pi, \tilde{\pi})$ as the cost of executing $\pi$ for one time step, and then executing $\tilde{\pi}$ for $t-1$ time steps. 

We will assume the cost-to-go difference between the learned policy and the optimal policy for task $k$ is bounded: $Q_t^k(\bx, \pith, \pi^*) - Q_t^k(\bx, \pi^*, \pi^*) \leq \delta \forall k$. This can be ensured by assuming universality of meta-learning.

% In the worst case, $\delta$ is $O(T)$ and \plato (as well as similar methods such as DAgger) will not outperform supervised learning. However, if $\pi^*$ is able to quickly recover from mistakes made by $\pith$, $\delta$ will be $O(1)$~\cite{Ross2011_AISTATS}.

[TODO talk about the mixture policy]
% When optimizing Equation \ref{eqn:obj} to obtain the teacher policy $\pila$, we choose $\lambda$ such that $\dkl(\pila(\bu | \bx) || \pith(\bu | \bo)) \leq \epslt$ for all state-observation pairs $(\bx, \bo)$. We can always guarantee this bound when optimizing Equation \ref{eqn:obj}  because $\dkl(\pila(\bu | \bx) || \pith(\bu | \bo)) \rightarrow 0$ as $\lambda \rightarrow \infty$.

When optimizing the supervised learning objective in the outer loop of meta-optimization [cite] to obtain the meta-learned policy initialization $\pith$, we assume the supervised learning objective function error is bounded by a constant $\dkl(\pith + \nabla_k \pith || \pi_k^*) \leq \epsts$ for all tasks $k$ and all per-task expert policies $\pi_k^*$. This bound essentially corresponds to assuming that the meta-learner attains bounded training error, which follows from the universality property proven in [cite Finn]. 

Let $l_k(\bx, \pith + \nabla_k \pith, \pi_k^*)$ denote the expected 0-1 loss of $\pith + \nabla_k \pith$ with respect to $\pi_k^*$ in state $\bx$: $\E_{\bu_\theta \sim (\pith + \nabla_k \pith)(\bu | \bx), \bu^* \sim \pi_k^*(\bu | \bx)} [ \mathbf{1}[\bu_\theta \neq \bu^*]]$. From prior work [], we know that the total variation divergence is an upper bound on the 0-1 loss  \cite{Nguyen2005_NIPS} and KL-divergence is an upper bound on the total variation divergence \cite{Pollard2000}. 

Therefore, the 0-1 loss can be upper bounded:
\begin{align*}
l_k(\bx, \pith + \nabla_k \pith, \pi_k^*) &= \E_{\bu_\theta \sim (\pith + \nabla_k \pith)(\bu | \bx), \bu^* \sim \pi_k^*(\bu | \bx)} [ \mathbf{1}[\bu_\theta \neq \bu^*]] \\
&\leq \dtv(\pith + \nabla_k \pith || \pi_k^*) \\
&\leq \sqrt{\dkl(\pith + \nabla_k \pith || \pi_k^*)} \\
&\leq \sqrt{\epsts}.
\end{align*}

% We also note the state distribution bound $||d_\pi^t - d_{\tilde{\pi}}^t||_1 \leq 2 t \sqrt{\dklmax(\pi, \tilde{\pi})}$ proven in \cite{Schulman2015_ICML}. This lemma implies that for an arbitrary function $f(\bx)$, $E_{\bx \sim d_\pi^t}[f(\bx)] \leq E_{\bx \sim d_{\tilde{\pi}}^t}[f(\bx)] + 2 f^{\max} t \sqrt{\dklmax(\pi, \tilde{\pi})}$

This allows us to bound the meta-learned policy performance using the following theorem: 

\begin{theorem}
Let the cost-to-go $Q_t^k(\bx, \pith + \nabla_k \pith, \pi_k^*) - Q_t^k(\bx, \pi_k^*, \pi_k^*) \leq \delta$ for all $t \in \{1, ..., T\}, k \sim p(\text{tasks})$ . Then in \textnormal{GMPS}, $J(\pith + \nabla_k \pith) \leq J(\pi_k^*) + \delta \sqrt{\epsts} O(T)$, and by extension $\mathbb{E}_{k \sim \text{tasks}}[J(\pith + \nabla_k \pith)] \leq \mathbb{E}_{k \sim \text{tasks}}[J(\pi_k^*)] + \delta \sqrt{\epsts} O(T)$
\label{theorem:mgps}
\end{theorem}

\noindent \textit{Proof}:
{\small
\begin{subequations}
\begin{align}
\!\!\!\!J(\pith)
&= J(\pi^*) + \sum_{t=0}^{T-1} J_{t+1}(\pith, \pi^*) - J_{t}(\pith, \pi^*) \nonumber \\
&= J(\pi^*) + \sum_{t=1}^T \E_{\bx \sim d_{\pith}^t}[Q_{t}(\bx, \pith, \pi^*) - Q_{t}(\bx, \pi^*, \pi^*)] \nonumber \\
&\leq J(\pi^*) + \delta \sum_{t=1}^T \E_{\bx \sim d_{\pith}^t} [ l(\bx, \pith, \pi^*) ] \label{eq:proof-loss} \\
&\leq J(\pi^*) + \delta \sum_{t=1}^T \E_{\bx \sim d_{\pila}^t} [ l(\bx, \pith, \pi^*) ] \!+\! 2 l^{\max} t \sqrt{\epslt} \label{eq:proof-dist} \\
&\leq J(\pi^*) + \delta \sum_{t=1}^T \sqrt{\epsts} + 2 t \sqrt{\epsts} \sqrt{\epslt} \label{eq:proof-loss-upper} \\
&= J(\pi^*) + \delta T \sqrt{\epsts} + \delta T (T+1) \sqrt{\epsts} \sqrt{\epslt} \nonumber
\end{align}
\end{subequations}
}%
Equation \ref{eq:proof-loss} follows from the fact that the expected 0-1 loss of $\pith$ with respect to $\pi^*$ is the probability that $\pith$ and $\pi^*$ pick different actions in $\bx$; when they choose different actions, the cost-to-go increases by $\leq \delta$. Equation \ref{eq:proof-dist} follows from the state distribution bound proven in \cite{Schulman2015_ICML}. Equation \ref{eq:proof-loss-upper} follows from the upper bound on the 0-1 loss.

Although we do not get to choose $\epsts$ because that is a property of the supervised learning algorithm and the data, we are able to choose $\epslt$ by varying parameter $\lambda$. If we choose $\lambda$ such that $\epslt = O(\frac{1}{T^2})$. We therefore have

% \begin{align*}
% J(\pith) \leq J(\pi^*) + \delta \sqrt{\epsts} O(T) + O(1) \hspace{0.1in} \tag*{$\square$}.
% \end{align*}

As with DAgger, in the worst case $\delta = O(T)$. However, in many cases $\delta = O(1)$ or is sub-linear in $T$, for instance if $\pi^*$ is able to quickly recover from mistakes made by $\pith$.
We also note that this bound, $O(T)$, is the same as the bound obtained by DAgger, but without actually needing to directly execute $\pith$ at training time. Compared to supervised learning with bound $O(T^2)$ \cite{Ross2011_AISTATS}, \plato trains the policy at states closer to those induced under its own distribution.
% \section{Convergence Proof}
% \label{sec:proof}

% \todo{work on notation, integrate this with the rest of the paper.}

% The overall multi-task meta-imitation algorithm is described below

% \begin{algorithm}[!h]
% \LinesNumbered
% \DontPrintSemicolon
% \SetAlgoLined
%  Initialize data buffer $D$\;
%  Initialize policy $\hat{\pi_1}$\;

%  \For{iteration $i$}{
%     \For{task $k$}{
%         $\pi_i^k = \beta_i\pi_k^* + (1-\beta_i)(\hat{\pi_i} + \nabla_k \hat{\pi_i})$\\
%         Sample $T$ step trajectories using $\pi_i^k$ \\
%         Get dataset $D_i^k = \{(s, \pi_k^*(s), k)\}$ \; \\
%         Aggregate datasets $D_i = \bigcup D_i^k$ \; \\
%         Train policy $\hat{\pi_{i+1}}$ using the meta-loss defined in Eqn [] and on dataset $D_i$.\\
%     }
%  }
%  Return best $\hat{\pi_i}$ on validation
% \caption{Meta-DAgger}
% \label{alg:metadagger}
% \end{algorithm}

% %%SL.1.20: Don't assume the reader knows what DAgger is, but also don't present it as a variant of DAgger. It's fine to cite DAgger and say that the proof is closely related, but it should stand on its own
% This algorithm is essentially following the paradigm of no regret follow the leader algorithms popular in online learning. It can be thought of as similar to the DAgger algorithm, but the loss function $\mathbb{E}_{s \sim d_{\pi}}(l(s, \pi))$ is replaced by $\mathbb{E}_{k \sim p(\text{tasks})} \mathbb{E}_{s \sim d_{\pi + \nabla_k \pi}}(l(s, \pi + \nabla_k \pi))$. This algorithm will converge to the optimal solution for every task under 2 assumptions: 
% \begin{enumerate}
%     \item $l(s, \pi + \nabla_k \pi)$ is strongly convex in $\pi$, $\forall s, k$. 
%     \item The universality property, i.e $\exists \pi, \mathbb{E}_{k \sim p(\text{tasks})} \mathbb{E}_{s \sim d_{\pi + \nabla_k \pi}}(l(s, \pi + \nabla_k \pi)) = \mathbb{E}_{k \sim p(\text{tasks})} \mathbb{E}_{s \sim d_{\pi_k^*}}(l(s, \pi_k^*))$, assuming an infinitely expressive class of function approximator.
%     %%SL.1.20: Phrase the second assumption differently: you are assuming *bounded training error*, you don't need *zero training error*! You can formally state what you want, and then explain how universality gets you this
% \end{enumerate}

% The convergence proof of this algoritihm can be given by the following

% \textbf{Theorem 1:} For GMPS, there exists a policy $\hat{\pi} \in \hat{\pi}_{1:N}$, s.t $\mathbb{E}_{k \sim p(\text{tasks})} \mathbb{E}_{s \sim d_{\hat{\pi} + \nabla_k \hat{\pi}}}(l(s, \hat{\pi} + \nabla_k \hat{\pi})) \leq \eps_N + \gamma_N + 2\frac{l_{\text{max}}}{N}\Bigg[n_{\beta} + T\sum_{j=n_\beta +1}^N \beta_j \Bigg]$
% %%SL.1.20: can we find a way to state the theorem so that it's a bit more concise? maybe wrap up all those bound terms into a symbol we can refer to? The key point in the theorem is that suboptimality is bounded by some number that decreases with epsilon, but this is not actually described...

% We define \\

% $\eps_N = \min_{\pi} \frac{1}{N} \sum_{i=1}^N \mathbb{E}_{k \sim p(\text{tasks})} \mathbb{E}_{s \sim d_{\pi_i^k}}(l(s, \pi + \nabla_k \pi))$ \\

% $\frac{1}{N}\sum_{i=1}^N \mathbb{E}_{k \sim p(\text{tasks})} \mathbb{E}_{s \sim d_{\pi_i^k}}(l(s, \hat{\pi_i} + \nabla_k \hat{\pi_i})) - \min_{\pi} \frac{1}{N}\sum_{i=1}^N \mathbb{E}_{k \sim p(\text{tasks})} \mathbb{E}_{s \sim d_{\pi_i^k}}(l(s, \pi + \nabla_k\pi)) \leq \gamma_N$

% $n_\beta$ is the largest $n < N$ such that $\beta_{n_{\beta}} > \frac{1}{T}$. 

% $l(s, \pi) \leq l_{\text{max}} \forall \pi$

% We can prove this by first proving lemma 1, which bounds the total variation distance as follows:

% %%SL.1.20: When writing out the proof, state the lemmas and prove them in the appendix. Try to avoid the alphabet soup -- maybe introduce a symbol for the post-update policy instead of constantly writing out the grad operator?
% \textbf{Lemma 1:} \\
% $\forall k, \|d_{\pi_i^k} - d_{\hat{\pi_i} + \nabla_k\hat{\pi_i}} \|_1 \leq 2T\beta_i$

% Let d be the probability that for task k, $\pi_i^k$ picks $\pi_k^*$ at least once in $T$ time steps. Then we can write 
% $d_{\pi_i^k} = (1-\beta_i)^T d_{\hat{\pi_i} + \nabla_k\hat{\pi_i}} + (1 - (1-\beta_i)^T)d$

% \begin{align}
%     \|d_{\pi_i^k} - d_{\hat{\pi_i} + \nabla_k\hat{\pi_i}} \|_1 &= (1 - (1- \beta_i)^T)\|d - d_{\hat{\pi_i} + \nabla_k\hat{\pi_i}}\|_1 \\ 
%     &\leq 2(1 - (1- \beta_i)^T) \\
%     &\leq 2T\beta_i
% \end{align}

% This lemma implies that $\mathbb{E}_{k \sim p(\text{tasks})} \mathbb{E}_{s \sim d_{\hat{\pi_i} + \nabla_k \hat{\pi_i}}}(l(s, \hat{\pi_i} + \nabla_k\hat{\pi_i})) \leq \mathbb{E}_{k \sim p(\text{tasks})} \mathbb{E}_{s \sim d_{\pi_i^k}}(l(s, \hat{\pi_i} + \nabla_k\hat{\pi_i})) + 2l_{\text{max}}\min(1, T\beta_i)$

% So now, we can prove theorem 1: 
% \begin{align}
%     &\min_{\hat{\pi} \in \hat{\pi}_{1:N}} \mathbb{E}_{k \sim p(\text{tasks})} \mathbb{E}_{s \sim d_{\hat{\pi} + \nabla_k \hat{\pi}}}(l(s, \hat{\pi} + \nabla_k\hat{\pi})) \\
%     & \leq \frac{1}{N} \sum_{i=1}^N \mathbb{E}_{k \sim p(\text{tasks})} \mathbb{E}_{s \sim d_{\hat{\pi_i} + \nabla_k \hat{\pi_i}}}(l(s, \hat{\pi_i} + \nabla_k\hat{\pi_i})) \\
%     & \leq \frac{1}{N} \sum_{i=1}^N \mathbb{E}_{k \sim p(\text{tasks})} \mathbb{E}_{s \sim d_{\pi_i^k}}(l(s, \hat{\pi_i} + \nabla_k\hat{\pi_i})) + 2l_{\text{max}}\min(1, T\beta_i)\\
%     & \leq \gamma_N + 2\frac{l_{\text{max}}}{N}\Bigg[n_{\beta} + \sum_{j=n_{\beta}+1}^N \beta_j\Bigg] + \\
%     & \min_{\pi} \frac{1}{N} \sum_{i=1}^N \mathbb{E}_{k \sim p(\text{tasks})} \mathbb{E}_{s \sim d_{\pi_i^k}}(l(s, \pi + \nabla_k\pi))\\
%     &= \eps_N + \gamma_N + 2\frac{l_{\text{max}}}{N}\Bigg[n_{\beta} + T\sum_{j=n_\beta +1}^N \beta_j\Bigg]
% \end{align}

% This ensure good performance under the error reduction assumption of DAgger,
% %%SL.1.20: don't refer to it as an assumption of dagger, refer to the actual place in the proof where you state the precise assumption
% the no regret conditions imposed by the FTL algorithm that we use and a careful choice of $\beta_i$, such that []. 

==> pseudocode.tex <==



\begin{algorithm}[t]
\caption{Meta Reinforcement Learning via Imitation (MRI)}
\label{alg:overview}
\begin{algorithmic}[1]
{\footnotesize
\REQUIRE $p(\task)$: distribution over tasks
\REQUIRE demonstrations $\data_{\task_i} \triangleq \{ \demo_j \}_i$ for each task $\task_i$
\REQUIRE $\alpha$, $\beta$: step size hyperparameters
\STATE randomly initialize $\theta$
\WHILE{not done}
    \STATE Sample task $\task_i \sim p(\task)$ \{or minibatch of tasks\}
    \STATE Sample $K$ trajectories $\data^\text{tr}=\{(\state_1,\action_1,...\state_H)\}$ using $\pi_\theta$ in $\task_i$
    \STATE $\theta_\text{init} \leftarrow \theta$
    \FOR{$n=1...N_\text{BC}$}
          \STATE Evaluate $\nabla_\theta \loss_\text{RL}(\theta, \data^\text{tr})$ according to  Eq.~\ref{eq:RLobj} and~\ref{eq:importance_sampling} with importance weights $\frac{\pi_\theta(\action_t | \state_t)}{\pi_{\theta_\text{init}}(\action_t | \state_t)}$
          \STATE Compute adapted parameters with gradient descent: $\phi_i=\theta-\alpha \nabla_\theta  \loss_{RL}( \theta, \data^\text{tr} )$
          %\STATE Sample trajectories $\mathcal{D}_i'=\{(\state_1,\action_1,...\state_H)\}$ using $f_{\theta_i'}$ in $\task_i$ 
          \STATE Sample demonstrations $\data^\text{val} \sim \data_{\task_i}$
          \STATE Update $\theta \leftarrow \theta - \beta \nabla_\theta  \loss_\text{BC} ( \phi_i, \data^\text{val})$ according to Equation~\ref{eq:bcobj}
     \ENDFOR
\ENDWHILE
}
%\STATE while 
\end{algorithmic}
\end{algorithm}
